Reasoning Pattern Matters: Learning to Reason without Human Rationales

Large Language Models (LLMs) have demonstrated remarkable reasoning capabilities under the widely adopted SFT+RLVR paradigm, which first performs Supervised Fine-Tuning (SFT) on human-annotated reasoning trajectories (rationales) to establish initial reasoning behaviors, then applies Reinforcement Learning with Verifiable Rewards (RLVR) to optimize the model using verifiable signals without golden rationales. However, annotating high-quality rationales for the SFT stage remains prohibitively expensive. This paper investigates when and how rationale annotation costs can be substantially reduced without compromising reasoning performance. We identify a broad class of problems, termed patterned reasoning tasks, where reasoning follows a fixed, procedural strategy consistent across instances. Although instances vary in content such as domain knowledge, factual information, or numeric values, the solution derives from applying a shared reasoning pattern. We argue that the success of SFT+RLVR on such tasks primarily stems from its ability to enable models to internalize these reasoning patterns. Using numerical semantic matching as a representative task, we provide both causal and behavioral evidence showing that reasoning patterns rather than the quantity or quality of rationales are the key determinant of performance. Building on these insights, we propose Pattern-Aware LLMs as Rationale AnnOtators (PARO), a simple yet effective framework that enables LLMs to generate rationales aligned with task-specific reasoning patterns without requiring human rationale annotations. Experiments show that PARO-generated rationales achieve comparable SFT+RLVR performance to human rationales that are 10 times larger. These results suggest that large-scale human rationale annotations can be replaced with LLM-based automatic annotations requiring only limited human supervision over reasoning patterns.

==> controlled_exps.tex <==
\section{Reasoning Pattern Matters}

In this section, we design controlled experiments to demonstrate that reasoning pattern serves as the key factor when leveraging rationales, outweighing two alternative factors: task-specific knowledge (Section~\ref{sec:task_specific_knowledge}) and label correctness (Section~\ref{sec:label_correctness}).

\subsection{Reasoning Pattern over Task-Specific Knowledge}\label{sec:task_specific_knowledge}

We aim to investigate whether reasoning pattern matters more than task-specific knowledge when leveraging rationales. To achieve this, we reduce the size of the RatQA-10k dataset by 10-fold, randomly retaining only 1k out of 10k training samples. Previous studies~\cite{jiang2025predicting} have shown that training dataset size is highly correlated with the volume of task-specific knowledge acquired. This reduction results in significantly lower task-specific knowledge while preserving the overall reasoning pattern present in each training sample.

We employ the same training recipe as SFT+RRFT described in Section~\ref{sec:implement_detail}. The results of SFT+RRFT (only 1k rationale samples) are presented in Table~\ref{tab:strategy-comparison}. The performance remains comparable to the full SFT+RRFT, with F1 decreasing by merely 1.2 points. This is particularly notable when compared to incentive-based methods, which lag significantly behind SFT+RRFT by 2.5-12.7 points. These results indicate that training dataset size is not the primary factor driving the performance gains of SFT+RRFT, thereby supporting our hypothesis that reasoning patterns are the crucial component.

\subsection{Reasoning Pattern over Label Correctness}\label{sec:label_correctness}

Previous work~\cite{min2022rethinking} has indicated that golden demonstrations are not strictly required for in-context learning—randomly replacing labels in demonstrations barely hurts the performance across a range of classification and multiple-choice tasks. In this section, we investigate whether this phenomenon extends to SFT+RRFT: specifically, whether the label correctness of rationales significantly impacts performance. 
To achieve this, we randomly replace 25\% of human-annotated rationales with incorrect rationales while maintaining the underlying reasoning pattern unchanged. We prompt GPT-4.1\footnote{gpt-4.1-2025-04-14} to modify 25\% of manually-annotated rationales into incorrect rationales. The detailed prompt is provided in Appendix C. 

We employ the same training recipe as SFT+RRFT described in Section~\ref{sec:implement_detail}. The results of SFT+RRFT (1k, 25\% wrong) are presented in Table~\ref{tab:strategy-comparison}. Remarkably, the performance of SFT+RRFT (1k, 25\% wrong) remains comparable to the full SFT+RRFT, with F1 decreasing by merely 0.7 points. 
These results demonstrate that label correctness of rationales is not the primary factor driving the performance gains of SFT+RRFT. Instead, they provide compelling evidence that reasoning patterns constitute the crucial component, consistent with findings from the in-context learning literature and further validating our central hypothesis.


\subsection{Analysis of Performance Gaps Between Training Phases}

\begin{figure*}[!tb]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/datasize_sft_rl.pdf}
        \caption{Impact of Dataset Size on the performance of SFT and RRFT phase. We report the results on annual report subset.}
        \label{fig:datasize-sft-rl}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/label_correct_sft_rl.pdf}
        \caption{Impact of label correctness on the performance of SFT and RRFT phase. We report the results on annual report subset.}
        \label{fig:label-correct-sft-rl}
    \end{minipage}
\end{figure*}

To better understand the roles of SFT and RRFT phases, we conduct a detailed analysis of intermediate performance under different rationale data conditions from Section~\ref{sec:task_specific_knowledge} and Section~\ref{sec:label_correctness}. Figure~\ref{fig:datasize-sft-rl} and Figure~\ref{fig:label-correct-sft-rl} present the performance comparison after each training phase across different evaluation metrics.

The results reveal two key insights about our SFT+RRFT training pipeline:

\textbf{SFT phase: Quantity and quality of rationales are critical.} During supervised fine-tuning, both the quantity and quality of rationales significantly impact model performance. The 10k SFT model substantially outperforms the 1k SFT model across all metrics (e.g., 59.4\% vs. 49.1\% F1 score), demonstrating that abundant rationale data provides richer task-relevant knowledge for establishing stronger initial reasoning capabilities. A similar pattern emerges in Figure~\ref{fig:label-correct-sft-rl} when comparing models trained with correct versus incorrect rationales (25\% wrong), where data quality directly translates to a 2\% F1 score degradation. These substantial gaps underscore the importance of rationale quantity and quality in building a solid foundation for reasoning.

\textbf{RRFT phase: Performance convergence through self improvement.} After RRFT training, the performance gaps nearly disappear, with final models achieving remarkably similar results—differences of only 0.9\% and 0.2\% in F1 score for the dataset size and label correctness experiments, respectively. This convergence indicates that RRFT can effectively compensate for initial weaknesses by learning task-relevant knowledge from large-scale (question, answer) pairs, even when starting from suboptimal SFT baselines. The key mechanism behind this robustness is that as long as the SFT phase establishes basic reasoning patterns—regardless of data limitations or quality issues—the model can continue to self-improve during RRFT by generating diverse rationales and reinforcing correct reasoning paths that lead to accurate answers while suppressing incorrect ones.

This complementary learning dynamic highlights the synergistic relationship between SFT and RRFT phases: \textbf{SFT provides essential reasoning patterns and templates, while RRFT enables scalable knowledge acquisition through self-exploration of the reasoning space.} This property makes the approach robust to limited availability of high-quality rationale data, a common challenge in real-world applications.




==> method.tex <==
\section{Methodology}
\subsection{Task Formulation}
Given two numerical mentions $n_1$ and $n_2$ with their corresponding contexts $c_1$ and $c_2$, numerical semantic matching (NSM) aims to determine whether the two mentions refer to the same underlying numerical fact—that is, whether they are semantically equivalent. Here, the context of a numerical mention encompasses the paragraph or table containing the mention along with its surrounding textual information, as illustrated in Figure \ref{fig:intro_example}. All contexts are converted to strings, with tables formatted using markdown syntax.

We formalize the NSM task as a question answering problem, following previous work~\cite{pang2025document}. Specifically, each question comprises the following three components: (1) \textbf{Task description} that provides detailed task instructions; (2) \textbf{Input context} that supplies the contexts $c_1$ and $c_2$, where numerical mentions are masked with placeholders to prevent LLMs from relying on value equality as shortcuts to determine semantic equivalence; (3) \textbf{Output instruction} that specifies the target mention pairs and their locations in the context, and instructs the model to make a binary decision on whether the two mentions are semantically equivalent. The answer format is ``yes/no'', indicating equivalent or not equivalent.

In this paper, we explore how to leverage rationales---human-annotated reasoning trajectories---to develop NSM reasoning capabilities. We investigate a practical data resource setting: the training set includes a large collection of question-answer pairs $\mathcal{D}_d = \{(q, a)\}$ and a small collection of question-rationale-answer triples $\mathcal{D}_r = \{(q, r, a)\}$, where $q$, $r$, and $a$ denote question, rationale, and answer, respectively. In real-world applications, while ground-truth answers $a$ can be obtained through straightforward annotation, rationales $r$ demand expert knowledge and careful annotation to ensure the quality of reasoning processes.

In the following sections, we first introduce a basic reinforcement learning method (Section~\ref{sec:rrft}), followed by a review of two representative approaches for leveraging rationales: enforcement-based methods (Section~\ref{sec:enforcement}) and incentive-based methods (Section~\ref{sec:incentive}). For each method, we present our tailored recipes specifically designed for the NSM task.


\subsection{Rule-based Reinforcement Fine-Tuning}~\label{sec:rrft}

We begin by introducing our basic \textbf{R}ule-based \textbf{R}einforcement \textbf{F}ine-\textbf{T}uning (RRFT) approach for the NSM task. RRFT can be viewed as a simplified variant of existing methods for bootstrapping LLM reasoning~\cite{hoffman2023training} or as a streamlined form of reinforcement learning with execution feedback~\cite{gehring2024rlef}. The core principle underlying RRFT is straightforward: the policy receives rewards only when its generated responses are verifiably correct. 
RRFT optimizes the following objective function:
\begin{equation}
    \max_{\pi_\theta} \mathbb{E}_{y \sim \pi_\theta(q)} [R_{\text{RRFT}}(q, y)] = [v(y, a) - \beta \text{KL}[\pi_\theta(y|q) \| \pi_{\text{ref}}(y|q)]],
\end{equation}
where $v$ is the verifiable reward function. This function takes as input a ground-truth answer $a$ and a model-generated response $y$, and determines whether the final answer extracted from the response matches $a$:
\begin{equation}
    v(y, a) = \begin{cases}
1 & \text{if } \text{extract}(y) = a, \\
0 & \text{otherwise.}
\end{cases}
\end{equation}
Here, $\text{extract}(\cdot)$ denotes the answer extraction function that parses the final binary "yes/no" decision from the generated response $y$. We utilize the DAPO~\cite{yu2025dapo} algorithm to optimize the RRFT objective.

\subsection{Enforcement-Based Methods}\label{sec:enforcement}

Enforcement-based methods utilize rationales as part of the target output to enforce the model to mimic specific reasoning behaviors. The target output can be enforced through either a supervised fine-tuning (SFT) objective~\cite{trung2024reft} or a reinforcement fine-tuning objective~\cite{fu2025srft}. In this paper, we adopt a simple \textsc{SFT + RRFT} approach and leave exploration of the latter direction for future work.

Specifically, we first warm up the policy's reasoning capabilities using the rationales dataset $\mathcal{D}_{r}$ by optimizing the following SFT objective:
\begin{equation}
    \theta^{(1)} = \arg\max_{\theta} \mathbb{E}_{(q,r,a) \sim \mathcal{D}_r} \left[\log \pi_\theta\left(f_e(r,a) \mid q\right)\right],
\end{equation}
where $f_e(r,a)$ assembles the rationale $r$ and the answer $a$ to form the desired output for question $q$. Subsequently, we use $\theta^{(1)}$ as the initial model parameters and optimize the model on $\mathcal{D}_{d}$ under an RRFT objective:
\begin{equation}
    \max_{\theta} \mathbb{E}_{(q,a) \sim \mathcal{D}_d}\mathbb{E}_{y \sim \pi_\theta(\cdot|q)}[R_{\text{RRFT}}(q, y)].
\end{equation}


\subsection{Incentive-Based Methods}\label{sec:incentive}

RRFT can be modeled as the task of finding a path from the root of the problem-solving tree to a leaf node that represents the correct answer~\cite{liu2025uft,guan2025rstar}. However, the problem-solving tree for real-world tasks, such as mathematical reasoning~\cite{guan2025rstar} and numerical semantic matching, typically contains an enormous number of nodes, making it challenging for an LLM to discover the correct path through exploration alone~\cite{zhao2024marco}. Moreover, only a small fraction of the leaf nodes correspond to correct answers, resulting in the well-known sparse reward problem~\cite{ladosz2022exploration}.

Incentive-based methods~\cite{xi2024training,liu2025uft} address these challenges by concatenating the question with a human-annotated rationale, referred to as the \texttt{hint}, to guide the model towards the correct answer. For the NSM task, we first convert $\mathcal{D}_r = \{(q, r, a)\}$ into $\mathcal{D}_r' = \{(q', a)\}$, where $q' = f_i(q, r)$ denotes the prompt generation of a new hinted question consisting of the original question and the rationale. Our prompt template of $f_i(\cdot, \cdot)$ is presented in Appendix C. Then we optimize the following objective:
\begin{equation}
    \max_{\theta} \mathbb{E}_{(q,a) \sim f_m(\mathcal{D}_r', \mathcal{D}_d)}\mathbb{E}_{y \sim \pi_\theta(\cdot|q)}[R_{\text{RRFT}}(q, y)]
\end{equation}
where $f_m(\mathcal{D}_r', \mathcal{D}_d)$ represents the combination of the two datasets. We introduce three combining strategies:
\begin{enumerate}
    \item \textbf{Warmup}: We use $\mathcal{D}_r'$ as a warmup stage and sequentially concatenate $\mathcal{D}_r'$ with $\mathcal{D}_d$: $\mathcal{D}_r' \oplus \mathcal{D}_d$.
    \item \textbf{Uniform}: We randomly mix $\mathcal{D}_r'$ and $\mathcal{D}_d$ to provide uniform guidance throughout the entire training process.
    \item \textbf{Curriculum}: We employ a curriculum learning strategy that gradually reduces both the proportion of hinted samples and the length of hints  within $\mathcal{D}_r'$. Specifically, we implement two complementary mechanisms: (1) \textbf{Proportion scheduling}. The proportion of samples from $\mathcal{D}_r'$ (with hints) is gradually decreased from an initial value $\alpha$ to 0 throughout the training process. (2) \textbf{Hint length scheduling}. For the $i$-th hint-augmented sample during training, we introduce a hyperparameter $p_i$ that determines the expected hint length as $p_i L_i$, where $L_i$ is the original hint length. The parameter $p_i$ follows a cosine annealing schedule, and the actual hint length is sampled from a binomial distribution $\text{Binomial}(L_i, p_i)$. This curriculum approach provides a smoother transition from hint-assisted learning to independent problem-solving.
\end{enumerate}

